Data Augmentation for Leaf Segmentation and Counting Tasks in Rosette Plants

Deep learning techniques involving image processing and data analysis are constantly evolving. Many domains adapt these techniques for object segmentation, instantiation and classification. Recently, agricultural industries adopted those techniques in order to bring automation to farmers around the globe. One analysis procedure required for automatic visual inspection in this domain is leaf count and segmentation. Collecting labeled data from field crops and greenhouses is a complicated task due to the large variety of crops, growth seasons, climate changes, phenotype diversity, and more, especially when specific learning tasks require a large amount of labeled data for training. Data augmentation for training deep neural networks is well established, examples include data synthesis, using generative semi-synthetic models, and applying various kinds of transformations. In this paper we propose a method that preserves the geometric structure of the data objects, thus keeping the physical appearance of the data-set as close as possible to imaged plants in real agricultural scenes. The proposed method provides state of the art results when applied to the standard benchmark in the field, namely, the ongoing Leaf Segmentation Challenge hosted by Computer Vision Problems in Plant Phenotyping.

==> zz_alon_notes.tex <==

{\bf\em AZ notes}
{\bf\em AZ I think the INTRODUCTION should start with  "general" issues on data augmentation, image synthesis, etc. and the RELATED WORK contain a survey on data augmentation intended for leaves and Arabidopsis.
\\ Cover the following:
\\ object instantiation, segmentation, detection, localization 
\\ DL for plant phenotyping
\\ CVPPP database
\\ other database - avocado, banana
\\ our contribution - photo-realistic augmentation preserving geometric structure and texture
\\ simple vs. smart ("in the wild" vs. "data-specific" / "na\"{i}ve" vs "sophisticated") augmentation
\\ our results - currently 1st in LSC/LCC 
\\ Our rank in LSC/LCC: we see submissions only from 08/2018. 
\\ Several papers report higher ranks (especially in counting).
\\ But - the test set and the evaluation script were modified some time ago,
\\ A4 training set was inserted later than A1,A2,A3,
\\ and some papers report results on a sub-set (A1 only, etc.),
\\ or their results on a partial test-set.
\\ :) Few works report results on A5. We do.}

{\bf\em AZ: Description of the CVPPP dataset - creation, importance, type of plants, A1-A4 categories ,...cite all articles in the "terms and conditions"...insert here 2-3 "fine-grained" sentences on the database !!}\\

% Related Efforts
%Several works propose data augmentation by synthesizing leaf images.
%The main approaches include {\em Graphical Modelling}, {\em Domain Randomization} (randomizing parameters such as lighting, pose, textures), and {\em Generative Adversarial Networks} in various forms. 
% branch their ideas from three stems...
%The DL/AI revolution is ... apparent in ... recent approaches to tackle ... trying various ways ... for data augmentation by synthesizing leaf images...  

\\{\bf\em AZ: collages in the computer vision / graphics literature}

\\{\bf\em\ AZ: the GAN paragraph is a mess
\\ go back to the articles and google
\\ rephrase
\\ 
\\ GANS are ... condition is... 
\\ some wiseguy did a arabidopsis-out-of-the-hat trick 
\\ then another fellow done a ARA synth with GANs
\\ 
\\ }
{\bf\em\ AZ:  Giuffrida 
\\ DCGAN, 
\\ condition - number of leaves, inserted to all/most of the Generator's layers.
\\ Generator: input - random noise (!!!), output - 128x128 RGB simulated ARA ("so called")
\\ Discriminator: mirror of the Generator's architecture, outputs binary decision on num leaves
\\ used their earlier work to count ARA leaves 
\\ The magic:
\\ start with random noise, and a condition (num leaves)
\\ and roll the dice until you get 128x128 RGB with greenish blobs that score high on the LCC
\\ 
}

\\{\bf\em\ AZ:  Zhu is a good one. 
\\ masks are generated in a structured manner.
\\ the cGAN does the magic of replacing mask image with RGB image
\\ addresses the COUNT, uses A4,Ax
\\ also uses MaskRCNN just for evaluation.
}

{\bf\em AZ: this is the place for a short summary of related work.
\\ put a short comparison of pros/cons of the surveyed approaches.
\\ the relevant ones (have smart synth, high results, potential for easy upgrade ...)
\\ still want the criticism ??
\\
\\ summary:
\\ good/bad for plant phenotyping 
\\ W/WO potential for extension to other datasets - 
\\ W/WO connection to real-world phenomena (measurable traits- area, shape, ) 
\\ all those proud of counting are missing the point. fancy acrobatics (we also want it) , but worthless if only applicable to guessing number of leaves in a snapshot.
}

{\bf\em AZ: METHODS:
\\remember to relate described methods to related work: graphical modelling of leaves, random params,  NNs.
\\Try to list and explain our advantages
\\ basic (na\"{i}ve) collage - for "in the wild conditions", or minimal collection of data and annotations, and still expecting to do some predictions.
\\ smart (structured) collage - for advanced blabla when certain structures are assumed/formalized/known to be correlated to the real world... }
{\bf\em AZ: first a short description and then details such as parameters...}
{\bf\em AZ: reference the "pipeline" figure}
{\bf\em AZ: do you want to expand and include:
\\the triads? leaves come in threes...
\\or approx 120 degrees +- epsilon
\\or separation into groups of small/medium/large sized leaves
}

{\bf\em AZ: maybe \(T_i (I,l,\alpha) \) or  \(T_i (I,l,f(\alpha)) \) , because \(T\) is also a function of the angle}\\
{\bf\em AZ:  \(T_0\) is an initialization, not a function \(T\). also - define \(T_0\) in words, because it appears later}\\
{\bf\em AZ: don't like the \(F(T)\) }\\
{\bf\em AZ OK - this is the \(f(\alpha)\) function... }\\

{\bf\em AZ: RESULTS:
\\Make a clear point about segmentation vs. counting. We target the SEG, count is an added value.
\\ NO attempt at regression, NO usage of ground-truth number of leaves, NO use of ground-truth leaf centers.
\\ TODO:
\\ tested on all five (A1-A5) categories
\\ a paragraph on LSC/LCC evaluation \cite{}
\\ mention: DICE (same as IOU), ABS diff in count
\\ specifics of evaluation
\\ table of results - output of LSC submission
\\ try to explain the meaning of the results (where and why are they good or poor)
\\ training on A1 only, vs. training each category separately
\\ benefit (or lack of it) when applying transparency correction
\\ some explanation of what we see in the figures
\\
\\ our low rank in count, because:
\\ our goal is segmentation
\\ didn't use ground-truth count, nor leaf centers
\\ transparency correction improved the count
\\ easy to "cheat" by using submission results ... 
}

{\bf\em AZ restriction on minimum number of leaves points to a weakness in counting, eliminating the babies  ... also can connect to explanation of results (as seen in  the Fig with segmentation results) kind of not only doing away with the babies, as they mature, they tend to forget their past ... because no pics of few small leaves in the training set.}

{\bf\em AZ: Appendix
%The network configurations are listed in Table \ref{tab:MaskRCNNDefaultParameters}.
%{\bf\em AZ: We don't  need this table if this is exactly the default vals in the github; we already %mention params we modified, and cite the github implementation ...}\\
\\We DO need to mention everything specific to our implementation - \\GPU capability, number of epochs, actual running time 
\\comparable statistics (do we have any?)
\\nice visual pics , ...}

\\{\bf\em AZ Question - Do we want this (or other) Acknowledgment ?}

{\bf\em END AZ notes}


